Quasi-stars and the Sch\"onberg-Chandrasekhar limit

The mechanism by which the supermassive black holes that power bright quasars at high redshift form remains unknown. One possibility is that ... the monolithic collapse of a massive protogalactic disc ... leads to the formation of a quasi-star: a growing black hole, initially of typical stellar-mass, embedded in a hydrostatic giant-like envelope. Quasi-stars are the main object of study in this dissertation. ... In Chapter 1, I introduce the problem posed by the supermassive black holes that power high-redshift quasars. ... In Chapter 2, I outline the Cambridge STARS code and the modifications that are made to model quasi-star envelopes. In Chapter 3, I present models of quasi-stars where the base of the envelope is located at the Bondi radius of the black hole. The black holes in these models are subject to a robust upper fractional mass limit of about one tenth. In addition, the final black hole mass is sensitive to the choice of the inner boundary radius of the envelope. In Chapter 4, I construct alternative models of quasi-stars by drawing from work on convection- and advection-dominated accretion flows ... The evolution of these quasi-stars is qualitatively different from those described in Chapter 3. ... [T]he core black holes are no longer subject to a fractional mass limit and ultimately accrete all of the material in their envelopes. In Chapter 5, I demonstrate that the fractional mass limit found in Chapter 3 ... is in essence the same as the Sch\"onberg-Chandrasekhar limit. The analysis demonstrates ... that limits exist under a wider range of circumstances than previously thought. A test is provided that determines whether a composite polytrope is at a fractional mass limit. In Chapter 6, I apply this test to realistic stellar models and find evidence that the existence of fractional mass limits is connected to the evolution of stars into the red giants.

==> title.tex <==
%\thispagestyle{empty}
%\cleardoublepage
\begin{titlepage}
\null\vfill
% \begin{center}
% %{\vspace*{5mm}}
% { \Huge {\bfseries {\Title{}}} \par}
% {\large \vspace*{25mm} 
% %{{\includegraphics[bb = 0 0 292 336, width=30mm]{cam}} \par} 
% {{\includegraphics[height=37mm]{cam_bw}}
% {\includegraphics[height=37mm]{ioa}}
% {\includegraphics[height=37mm]{eds_bw}} \par} 
% \vspace*{20mm}}
% {{\Large \Author{}} \par}{\large \vspace*{1ex}
% {{Institute of Astronomy} \par}\vspace*{1ex}
% {{and} \par}\vspace*{1ex}
% {{St Edmund's College} \par}\vspace*{1ex}
% {{University of Cambridge} \par}\vspace*{25mm}
% {{{This dissertation is submitted for the degree of}} \par}\vspace*{1ex}
% {\it {Doctor of Philosophy} \par}\vspace*{2ex}
% {\Date{}}}  \end{center}
\begin{center}
%{\vspace*{5mm}}
{ \Huge {{\Title{}}} \par}
%{ \Huge {\fontfamily{ptm}\selectfont {\Title{}}} \par}
{\large \vspace*{25mm} 
%{{\includegraphics[bb = 0 0 292 336, width=30mm]{cam}} \par} 
{{\includegraphics[height=37mm]{cam_bw}}
{\includegraphics[height=37mm]{ioa}}
{\includegraphics[height=37mm]{eds_bw}} \par} 
\vspace*{20mm}}
{{\large \Author{}} \par}{\normalsize \vspace*{1ex}
{{Institute of Astronomy} \par}\vspace*{1ex}
{{and} \par}\vspace*{1ex}
{{St Edmund's College} \par}\vspace*{1ex}
{{University of Cambridge} \par}\vspace*{25mm}
{{{This dissertation is submitted for the degree of}} \par}\vspace*{1ex}
{\it {Doctor of Philosophy} \par}\vspace*{2ex}
%{\Date{}}
}\end{center}
\null\vfill
\end{titlepage}

